Irradiation-driven Evaporation of Micro Droplets in an Optical Trap

Small droplets are irradiated with visible and infrared light in many natural and industrial environments. One of the simplest ways to describe their evaporation is the D$^2$-Law. It states that the evaporation rate is proportional to $t^{-1/2}$, and $R^{-1}$. However, models like the D$^2$-Law do not account for the volumetric heating of light and the effect of strong irradiation on individual droplets is not fully understood. Here we show the effects of IR irradiation on optically levitated water droplets. We find that, under strong irradiation of up to $10^8 W/m^2$, the droplet evaporation is initially driven by the heat from the laser following the power law $dR / dt \sim R$, i.e. the inverse of the D$^2$-Law. Then, when the droplets shrink to 2 - 3 $\mu$m in radius a turnover occurs from irradiation-driven back to diffusion-driven evaporation. Our findings support the understanding of droplet evaporation in cases such as rocket engines or internal combustion, where the radiation from the flame will heat water and fuel droplets.

==> Sections/AnalogyToEnviromentalHeating.tex <==

\subsection{Analogous effects of NIR irradiation and Ambient temperature}
As shown in the theory section, the evaporation constant \(K\) typically ranges from \(10^{-11}\) to \(10^{-10}\) under ambient temperatures of 25 to 55~°C and a relative humidity of 98.6\% (Fig. 1). Our experiments revealed a similar trend (Fig. 8), where \(K\) varied from \(10^{-11}\) to \(10^{-10}\) as IR power increased from 0 to 100~mW, while maintaining a constant ambient temperature of 24.6~°C and a relative humidity of 98.6\%. 

This shows that we have an analogous behavior of IR power (irradiation on droplet) and ambient temperatures on the evaporation rates of the single component water droplet. 

\vspace{1em} % Add space before the figure


\vspace{-1em} % Add space after the figure

\vspace{1em} % Add space before the figure

\begin{figure}[H]
\centering
\includegraphics[width=\columnwidth]{Analogy_K_vs_Power (Experimental).jpg}
\caption{\textit{Analogous effects of IR irradiation power and ambient temperature (\(T_a\)) on the evaporation constant (K). The graph features a single y-axis with two x-axes: the upper x-axis shows IR power (in mW) with experimental data fitted using a logarithmic curve, while the lower x-axis displays ambient temperature (\(T_a\), in °C) with the fit from fig. The closeness of the experimental fit and theoretical predictions suggests a similar analogy of both of them on the evaporation process}}
\end{figure}

\vspace{-1em} % Add space after the figure.
According to the revised D\textsuperscript{2} law \cite{dallabarba2021}, the droplet reaches an asymptotic temperature (\(T_{ds}\)) that is typically lower than the ambient temperature (\(T_a\)). This asymptotic temperature corresponds to the wet-bulb temperature of the surroundings, which represents the lowest temperature to which air can be cooled by the evaporation of water at constant pressure. Therefore, under ideal conditions with no internal heating, \(T_{ds}\) should be less than \(T_a\). At higher humidity levels, \(T_{ds}\) approaches \(T_a\), but it cannot exceed \(T_a\) under ordinary conditions.

However, in our experiments, the application of infrared (IR) irradiation introduces internal heating of the droplet as discussed in the theory section. As a result, the thermal equilibrium during the evaporation process shifts, leading to a slight increase in the asymptotic droplet temperature (\(T_{ds}\)) compared to the usual wet-bulb temperature. Using the equations of the revised D\textsuperscript{2} law \cite{dallabarba2021}, we estimated this increase and observed (Fig. 9) that \(T_{ds}\) rises by approximately 1~°C above the ambient temperature (\(T_a\)) of 24.6~°C in the same ranges of \(K\) constant in our experiments and we see that the increase in NIR irradiation increases the droplet asymptotic temperature (\(T_{ds}\)).

\vspace{5em}

\begin{figure}[H]
\centering
\includegraphics[width=\columnwidth]{Tds vs Power.jpg}
\caption{\textit{Slight increase in the droplet asymptotic temperature \(T_{ds}\) above the ambient temperature of 24~°C with increase in NIR irradiation on the droplet.}}
\end{figure}
